Spatially Visual Perception for End-to-End Robotic Learning

Recent advances in imitation learning have shown significant promise for robotic control and embodied intelligence. However, achieving robust generalization across diverse mounted camera observations remains a critical challenge. In this paper, we introduce a video-based spatial perception framework that leverages 3D spatial representations to address environmental variability, with a focus on handling lighting changes. Our approach integrates a novel image augmentation technique, AugBlender, with a state-of-the-art monocular depth estimation model trained on internet-scale data. Together, these components form a cohesive system designed to enhance robustness and adaptability in dynamic scenarios. Our results demonstrate that our approach significantly boosts the success rate across diverse camera exposures, where previous models experience performance collapse. Our findings highlight the potential of video-based spatial perception models in advancing robustness for end-to-end robotic learning, paving the way for scalable, low-cost solutions in embodied intelligence.

==> sec/6_discussion.tex <==
% \section{Discussion}
% The findings presented in this paper highlight the potential of leveraging spatial data with corrupted RGB data to improve the robustness of robotic learning under varied lighting conditions, where the proposed method greatly outperformed other methods tested. This demonstrates particular value for real-world applications in settings with uncontrolled lighting, such as industrial or household environments.

% The observed performance degradation around exposure level 10 in the CupStack task (see Table \ref{tab:success_rates}) can be attributed to present noise in the generated policy trajectories under specific world states during testing. This noise interfered with task completion, especially in low-light conditions, where the model demonstrated difficulty in maintaining the correct sequence for completing tasks. 

% Notably for CupStack, the model's reliance on depth information in these conditions likely contributed to its inability to accurately distinguish between individual cups, resulting in errors in task order. These findings suggest that while depth-based cues offer value in low-light scenarios, they are insufficient for tasks requiring precise object identification and sequencing. Further optimization may involve enhancing visual feature extraction to improve object recognition under varying lighting conditions, thereby enabling more reliable performance in tasks with sequential dependencies.

% The results indicate a more gradual performance decline in models trained on PickBig and PickSmall tasks compared to CupStack (see Table \ref{tab:success_rates}). This discrepancy can likely be attributed to the smaller state space in PickBig and PickSmall, where minimal deviations in initial positions during training led the model to over-rely on robot pose data. Consequently, the model learned to depend on the robot arm's state to generate policy trajectories, resulting in limited generalizability. As a result, it struggled to differentiate between large and small blocks and exhibited reduced robustness to slight variations in initial block positions. This highlights the need for diverse initial conditions and state representations in training to improve model adaptability in environments with subtle spatial changes.
